Relational Models of Microarchitectures for Formal Security Analyses

There is a growing need for hardware-software contracts which precisely define the implications of microarchitecture on software security-i.e., security contracts. It is our view that such contracts should explicitly account for microarchitecture-level implementation details that underpin hardware leakage, thereby establishing a direct correspondence between a contract and the microarchitecture it represents. At the same time, these contracts should remain as abstract as possible so as to support efficient formal analyses. With these goals in mind, we propose leakage containment models (LCMs)-novel axiomatic security contracts which support formally reasoning about the security guarantees of programs when they run on particular microarchitectures. Our core contribution is an axiomatic vocabulary for formally defining LCMs, derived from the established axiomatic vocabulary used to formalize processor memory consistency models. Using this vocabulary, we formalize microarchitectural leakage-focusing on leakage through hardware memory systems-so that it can be automatically detected in programs. To illustrate the efficacy of LCMs, we present two case studies. First, we demonstrate that our leakage definition faithfully captures a sampling of (transient and non-transient) microarchitectural attacks from the literature. Second, we develop a static analysis tool based on LCMs which automatically identifies Spectre vulnerabilities in programs and scales to analyze realistic-sized codebases, like libsodium.

==> benchmark.tex <==
\newcommand{\yes}[]{\cmark}
\newcommand{\no}[]{\xmark}
\newcommand{\unk}[]{\~}

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
    {\it Benchmark} & {\it Spectre v1} & {\it Additional leakage} \\\hline
     PHT01 & \yes & \yes \\\hline
     PHT02 & \yes & \yes \\\hline
     PHT03 & \yes & \yes \\\hline
     PHT04 & \yes & \yes \\\hline
     PHT05 & \yes & \yes \\\hline
     PHT06 & \yes & \yes \\\hline
     PHT07 & \no & \yes \\\hline
     PHT08 & \yes & \yes \\\hline
     PHT09 & \yes & \yes \\\hline
     PHT10 & \no & \yes \\\hline
     PHT11 & \no & \yes \\\hline
     PHT12 & \yes & \yes \\\hline
     PHT13 & \no & \yes \\\hline
     PHT14 & \yes & \yes \\\hline
     PHT15 & \yes & \yes \\\hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
    {\it Benchmark} & {\it Spectre v4} & {\it Additional leakage} \\\hline
     STL01 &      \unk & \unk \\\hline
     STL02 &      \unk & \unk \\\hline
     STL03 &      \unk & \unk \\\hline
     STL04 &      \unk & \unk \\\hline
     STL05 &      \unk & \unk \\\hline
     STL06 &      \unk & \unk \\\hline
     STL07 &      \unk & \unk \\\hline
     STL08 &      \unk & \unk \\\hline
     STL09\_bis & \unk & \unk \\\hline
     STL10 &      \unk & \unk \\\hline
     STL11 &      \unk & \unk \\\hline
     STL12 &      \unk & \unk \\\hline
     STL13 &      \unk & \unk \\\hline
     STL14 &      \unk & \unk \\\hline
     \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}



==> checkmate-ref.tex <==
@INPROCEEDINGS{fmcad18, 
author={Hongce Zhang and \textbf{Caroline Trippel} and Yatin Manerkar and Aarti Gupta and Margaret Martonosi and Sharad Malik}, 
booktitle={2018 Formal Methods in Computer-Aided Design (FMCAD)}, 
title={Integrating Memory Consistency Models with Instruction-Level Abstraction for Heterogeneous System-on-Chip Verification}, 
year={2018}, 
volume={}, 
number={}, 
ISSN={}, 
month={October-November},}

@inproceedings{micro18,
 author = {\textbf{Caroline Trippel} and Daniel Lustig and Margaret Martonosi},
 title = {{CheckMate}: Automated Exploit Program Generation for Hardware Security Verification},
 booktitle = {51st International Symposium on Microarchitecture (MICRO)},
 year = {2018},
} 

@misc{intel18,
  title={Security Exploit Analysis and Synthesis: Formal Specifications and Model Finding Techniques},
  author={\textbf{Caroline Trippel} and Margaret Martonosi},
  year={2018},
  month=September,
  publisher={Intel Grant},
  note={\$100,000 per year for 3 years}
}

@article{arxiv18,
  author    = {\textbf{Caroline Trippel} and
               Daniel Lustig and
               Margaret Martonosi},
  title     = {{MeltdownPrime} and {SpectrePrime}: Automatically-Synthesized Attacks
               Exploiting Invalidation-Based Coherence Protocols},
  journal   = {ARXIV},
  volume    = {abs/1802.03802},
  year      = {2018},
  url       = {http://arxiv.org/abs/1802.03802},
  archivePrefix = {arXiv},
  eprint    = {1802.03802},
  timestamp = {Thu, 01 Mar 2018 15:00:45 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1802-03802},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@ARTICLE{toppicks18,
author = {\textbf{Caroline Trippel} and Manerkar, Yatin A. and Lustig, Daniel and Pellauer, Michael and Martonosi, Margaret},
journal={IEEE Micro}, 
title={Full-Stack Memory Model Verification with {TriCheck}}, 
year={2018}, 
volume={38}, 
number={3}, 
pages={58-68},
doi={10.1109/MM.2018.032271062}, 
ISSN={0272-1732}, 
month={May},}

@inproceedings{asplos17,
 author = {\textbf{Caroline Trippel} and Manerkar, Yatin A. and Lustig, Daniel and Pellauer, Michael and Martonosi, Margaret},
 title = {TriCheck: Memory Model Verification at the Trisection of Software, Hardware, and ISA},
 booktitle = {Proceedings of the Twenty-Second International Conference on Architectural Support for Programming Languages and Operating Systems},
 series = {ASPLOS '17},
 year = {2017},
 isbn = {978-1-4503-4465-4},
 location = {Xi'an, China},
 doi = {10.1145/3037697.3037719},
 acmid = {3037719},
} 

@article{arxiv16,
  author    = {Yatin A. Manerkar and \textbf{Caroline Trippel} and Daniel Lustig and Michael Pellauer and Margaret Martonosi. },
  title     = {Counterexamples and Proof Loophole for the {C/C++} to {POWER} and
               ARMv7 Trailing-Sync Compiler Mappings},
  journal   = {CoRR},
  volume    = {abs/1611.01507},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.01507},
  timestamp = {Thu, 01 Dec 2016 19:32:08 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/ManerkarTLPM16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{oakland16, 
author={Roberto Guanciale and Hamed Nemati and Christoph Baumann and Mads Dam}, 
booktitle={2016 IEEE Symposium on Security and Privacy (SP)}, 
title={Cache Storage Channels: Alias-Driven Attacks and Verified Countermeasures}, 
year={2016}, 
pages={38-55}, 
keywords={binary codes;cache storage;cryptography;safety-critical software;source code (software);trusted computing;128-bit key;AES encryption service;ARMv7 hypervisor;Raspberry Pi 2;TrustZone;alias-driven attacks;application processors;application security monitors;attack vector;cache access pattern;low-noise cache storage channel;mismatched memory attributes;security-critical services;security-critical software;self-modifying code;timing channel analysis techniques;trusted software binary code;virtual aliases;Cache storage;Monitoring;Program processors;Security;Timing;Virtual machine monitors;cache storage channels;hypervisor;side channels;verification}, 
doi={10.1109/SP.2016.11}, 
month={May},}

@INPROCEEDINGS{fmcad15, 
author={Pramod Subramanyan and Yakir Vizel and Sayak Ray and Sharad Malik}, 
booktitle={2015 Formal Methods in Computer-Aided Design (FMCAD)}, 
title={Template-based synthesis of instruction-level abstractions for SoC verification}, 
year={2015}, 
volume={}, 
number={}, 
doi={10.1109/FMCAD.2015.7542266}, 
ISSN={}, 
month={September},}

@inproceedings{isca15,
 author = {Lustig, Daniel and \textbf{Caroline Trippel} and Pellauer, Michael and Martonosi, Margaret},
 title = {{ArMOR}: Defending Against Memory Consistency Model Mismatches in Heterogeneous Architectures},
 booktitle = {42nd International Symposium on Computer Architecture (ISCA)},
 year = {2015},
} 

@inproceedings{lahav,
 author = {Lahav, Ori and Vafeiadis, Viktor and Kang, Jeehoon and Hur, Chung-Kil and Dreyer, Derek},
 title = {Repairing Sequential Consistency in {C/C++11}},
 booktitle = {Proceedings of the 38th ACM SIGPLAN Conference on Programming Language Design and Implementation},
 series = {PLDI 2017},
 year = {2017},
 isbn = {978-1-4503-4988-8},
 location = {Barcelona, Spain},
 pages = {618--632},
 numpages = {15},
 url = {http://doi.acm.org/10.1145/3062341.3062352},
 doi = {10.1145/3062341.3062352},
 acmid = {3062352},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {C++11, Weak memory models, declarative semantics, sequential consistency},
} 

